L2C2: Last-Level Compressed-Cache NVM and a Procedure to Forecast Performance and Lifetime

Several emerging non-volatile (NV) memory technologies are rising as interesting alternatives to build the Last-Level Cache (LLC). Their advantages, compared to SRAM memory, are higher density and lower static power, but write operations wear out the bitcells to the point of eventually losing their storage capacity. In this context, this paper presents a novel LLC organization designed to extend the lifetime of the NV data array and a procedure to forecast in detail the capacity and performance of such an NV-LLC over its lifetime. From a methodological point of view, although different approaches are used in the literature to analyze the degradation of an NV-LLC, none of them allows to study in detail its temporal evolution. In this sense, this work proposes a forecast procedure that combines detailed simulation and prediction, allowing an accurate analysis of the impact of different cache control policies and mechanisms (replacement, wear-leveling, compression, etc.) on the temporal evolution of the indices of interest, such as the effective capacity of the NV-LLC or the system IPC. We also introduce L2C2, a LLC design intended for implementation in NV memory technology that combines fault tolerance, compression, and internal write wear leveling for the first time. Compression is not used to store more blocks and increase the hit rate, but to reduce the write rate and increase the lifetime during which the cache supports near-peak performance. It has affordable hardware overheads compared to that of a baseline NV-LLC without compression in terms of area, latency and energy consumption, and increases up to 6-37 times the time in which 50\% of the effective capacity is degraded, depending on the variability in the manufacturing process.

==> RelatedWork.tex <==
%!TEX root = main.tex
\section{Related work}
\subsection{On enhancing NVM lifetime}

%Diversos trabajos en la literatura proponen mejorar la esperanza de vida de las NVM. Estos estudios se centran en, a) reducir el número de escrituras, b) adoptar algún mecanismo de redundancia o corrección de errores, o c) homogeneizar las escrituras sobre toda la estructura NVM.

Several works propose to improve NVM lifetime focusing on either a) reducing the number of writings, or b) adopting some redundancy or error correction mechanism, or c) distributing writes uniformly through the entire NVM structure.

%En primer lugar, existen diferentes mecanismos para reducir el número de escrituras que sufren las NVM \cite{Choi-17-NVMWayAllocation} \cite{Rodriguez-18-Reuse}. La compresión de datos, que es un ejemplo de ellos, puede integrarse en el contexto de memoria principal \cite{Dgien-14-CompressionArchitecture} \cite{Palangappa-18-CASTLE} \cite{Jadidi-17-CollaborativeCompression} o de la NV-LLC \cite{Choi-14-AdaptiveCacheCompression} \cite{Yazdanshenas-13-CodingLLC}. El denominador común de estos trabajos radica en utilizar la compresión para reducir el tamaño del bloque y, por consiguiente, reducir el número de bytes escritos en los contenedores. Este trabajo, al igual que \cite{Ferreron-15-Concertina} \cite{Jadidi-17-CollaborativeCompression}, sugiere una segunda perspectiva: permitir que los contenedores con celdas defectuosas puedan albergar bloques comprimidos.

First, there are several mechanisms to reduce the number of writes NVMs suffer \cite{Choi-17-NVMWayAllocation} \cite{Rodriguez-18-Reuse} \cite{Wang-14-AdaptivePlacementHybrid}. As an example, data compression can be integrated into the main memory or the NV-LLC context \cite{Dgien-14-CompressionArchitecture} \cite{Palangappa-18-CASTLE} \cite{Jadidi-17-CollaborativeCompression} \cite{Choi-14-AdaptiveCacheCompression} \cite{Yazdanshenas-13-CodingLLC}. These works share the use of compression to reduce the block size and, consequently, reduce the number of bytes written to the frames. This work, like \cite{Ferreron-15-Concertina} \cite{Jadidi-17-CollaborativeCompression}, suggests a second insight: allowing frames with faulty cells to hold compressed blocks.

%En segundo lugar, para detectar y tolerar fallos en las celdas de memoria NVM es imprescindible adoptar algún mecanismo basado en códigos de detección y corrección de errores (ECC) \cite{Schechter-10-UseECPnotECC} \cite{Seong-10-SAFER} \cite{Ipek-10-DynamicallyReplicatedMemory} \cite{Yoon-11-FREE-p}. Por ejemplo, Schechter et al. proponen ECP, un mecanismo de ECC que codifica la ubicación de las celdas defectuosas y les asigna bitcells sanas para reemplazarlas \cite{Schechter-10-UseECPnotECC}. El inconveniente que presenta este mecanismo es que sólo puede soportar un número limitado de bitcells defectuosas (dependiente del sobrecoste).

Second, in order to detect and tolerate faults in NVM cells, it is essential to adopt some mechanism based on error detection and correction codes (ECC) \cite{Schechter-10-UseECPnotECC} \cite{Seong-10-SAFER} \cite{Ipek-10-DynamicallyReplicatedMemory} \cite{Yoon-11-FREE-p}. For instance, Schechter et al. propose ECP, an ECC mechanism that encodes the location of defective cells and assigns healthy bitcells to replace them \cite{Schechter-10-UseECPnotECC}. The drawback of this mechanism is that it can only support a limited number of faulty bitcells (overhead dependent).

%Por último, hay propuestas que se centran en homogeneizar el número de escrituras entre todas las celdas de la NV-LLC utilizando técnicas de \textit{wear-leveling} en todas las dimensiones fundamentales de la estructura de memoria: bancos, conjuntos, vías y bytes dentro de contenedor para el caso de una NV-LLC \cite{Wang-13-I2WAP} \cite{Farbeh-16-FloatingECC} \cite{Agarwal-20-LinovoThesis}.

Finally, some other proposals focus on uniforming the number of writings between all memory cells using \textit{wear-leveling} techniques in all the underlying dimensions of the memory structure: banks, sets, ways and bytes within a frame for the case of an NV-LLC \cite{Wang-13-I2WAP} \cite{Farbeh-16-FloatingECC} \cite{Agarwal-20-LinovoThesis}.

%Cualquiera de estas técnicas son ortogonales a nuestra propuesta y se integrarían de forma independiente. Nuestro procedimiento de pronóstico asume que la NV-LLC implementa dos técnicas de wear-leveling para distribuir las escrituras de forma uniforme tanto entre conjuntos como entre bytes de un contenedor. Además, supone un mecanismo SECDED capaz de corregir un error de la celda que se convierte en defectuosa.

Any of these techniques are orthogonal to our and would be integrated on a standalone basis. Our forecasting procedure assumes that the NV-LLC adopts two wear-leveling techniques to evenly distribute writes between sets and bytes within a frame. Furthermore, it assumes a SECDED mechanism able to correct an error in a faulty cell.


\subsection{On forecasting procedures}

%La mayoría de los trabajos anteriores usa la reducción relativa del número de escrituras como métrica para ilustrar la mejora en resistencia (\emph{endurance}) de las NVMs \cite{Choi-14-AdaptiveCacheCompression} \cite{Yazdanshenas-13-CodingLLC} \cite{Choi-17-NVMWayAllocation} \cite{Dgien-14-CompressionArchitecture} \cite{Palangappa-18-CASTLE}. Pero dicha métrica no sirve para conocer la evolución temporal de la capacidad efectiva de la cache ni de las prestaciones del sistema.

Most previous works use the relative reduction in the number of writes as a metric to depict the improvement in NVMs endurance \cite{Choi-14-AdaptiveCacheCompression} \cite{Yazdanshenas-13-CodingLLC} \cite{Choi-17-NVMWayAllocation} \cite{Dgien-14-CompressionArchitecture} \cite{Palangappa-18-CASTLE}. However, this metric is not suitable to know the temporal evolution of the effective capacity of the cache nor the performance of the overall system.

%Otros trabajos han propuesto un modelo simple de envejecimiento para analizar la evolución de la capacidad de una memoria principal NVM dotada de un mecanismo de deshabilitación de páginas completas \cite{Schechter-10-UseECPnotECC} \cite{Seong-10-SAFER} \cite{Yoon-11-FREE-p} \cite{Ipek-10-DynamicallyReplicatedMemory}. Estas propuestas modelan el número máximo de escrituras que soporta cada bitcell mediante una distribución normal con una media y un coeficiente de variación que depende de la tecnología NVM y del proceso de fabricación. Además, recopilan mediante simulación el número total de escrituras por unidad de tiempo y lo distribuyen entre todas las páginas de forma equitativa (asumen un \textit{inter-page wear-leveling}). Cuando el número de celdas defectuosas en una página es superior a lo que el sistema es capaz de soportar, la página se desactiva y las escrituras asociadas a ella se reparten equitativamente entre las demás \cite{Schechter-10-UseECPnotECC}.

Other works have proposed a simple aging model to analyze the capacity evolution of an NV main memory with a full-page disable mechanism \cite{Schechter-10-UseECPnotECC} \cite{Seong-10-SAFER} \cite{Yoon-11-FREE-p} \cite{Ipek-10-DynamicallyReplicatedMemory}. These proposals model the maximum number of writes supported by each bitcell using a normal distribution with mean and coefficient of variation depending on the NVM technology and the manufacturing process. In addition, they collect the total number of writes per unit time by simulation and equally distribute it over all pages (assuming an inter-page wear-leveling). When the number of defective cells on a page is higher than the system is able to support, the page is deactivated and the writes associated to it are evenly distributed among the others \cite{Schechter-10-UseECPnotECC}.

%El error principal de este modelo es ignorar la disminución en el número de escrituras por unidad de tiempo (ancho de banda de escritura) a medida que la memoria se degrada. En el contexto de memoria principal, esta degradación implica una disminución del número de contenedores de página disponibles y, en consecuencia, un aumento de los fallos de página y una disminución de las prestaciones. Esta pérdida de prestaciones provocará, a su vez, un cambio en la distribución y velocidad de las escrituras.

The main pitfall of this model falls to ignore the decrease in write bandwidth as memory degrades. In the main memory context, this degradation involves a decrease in the number of available page frames and, consequently, an increase in page faults and a decrease in performance. This loss of performance will, in turn, lead to a change in the distribution and speed of writes.

%Esta metodología sería fácilmente trasladable a una NV-LLC con Block-Disabling. Pero aquí, asumir que el ancho de banda de escritura agregado se mantiene constante en el tiempo, o asumir que las escrituras asociadas a un contenedor que se degrada se van a repartir equitativamente entre el resto de contenedores de la NV-LLC, no es correcto. 

This methodology would be easily applied to a NV-LLC with Block-Disabling. However, assuming that the aggregate write bandwidth remains invariant through time, or assuming that the writes associated with a degrading frame will be evenly distributed among the other frames in the NV-LLC, is not correct.

%Por un lado, la organización asociativa de la cache hace que las escrituras de un contenedor desactivado se deban repartir entre los contenedores del mismo conjunto, en lugar de entre todos los contenedores de la cache. Por otro lado, la degradación de la cache produce un aumento de la tasa de fallos lo que también provoca una pérdida de prestaciones que se traduce en una disminución del ancho de banda de escritura. Además, la desactivación de contenedores tampoco afecta igual a las prestaciones de las distintas aplicaciones puesto que el patrón de utilización de la NV-LLC de cada una de ellas puede ser muy distinto.

On the one hand, the associative nature of the cache means that writes from a disabled frame should be distributed among the rest of the frames in the same set, rather than among all the frames in the cache. On the other hand, cache degradation leads to an increase in the miss rate, which also results in a loss of performance which in turn translates into a decrease in write bandwidth. In addition, disabling frames does not affect the performance of different applications equally, since the NV-LLC usage pattern of each application may differ significantly.

%Finalmente, esta metodología no es aplicable en una NV-LLC con compresión. Dicha metodología se propuso para memorias cuyos contenedores tienen solo dos posibles estados: habilitado o deshabilitado. Cuando un contenedor se desactiva, el procedimiento asume que las escrituras que recibía se reparten de forma uniforme sobre el resto de la memoria. En una NV-LLC con compresión como la de nuestro trabajo, los contenedores pierden capacidad progresivamente. Al perder capacidad solamente dejan de recibir parte de sus escrituras. La cantidad de escrituras que dejan de recibir depende, entre otras cosas, del patrón de acceso de las aplicaciones y del factor de compresión de los bloques. Además, estas escrituras no se reparten uniformemente entre el resto de contenedores de la cache. Solo se reparten entre algunos de los contenedores que pertenecen al mismo conjunto: aquellos cuya capacidad efectiva es mayor que la del contenedor que se degrada.

Finally, this methodology cannot be applied to a compression-based NV-LLC. It was proposed for memories whose frames have only two potential states: enabled or disabled. When a frame is disabled, the procedure assumes that the writes it receives are evenly distributed through the rest of the memory. In a compression-based NV-LLC like the one in our work, the frames progressively lose capacity. Whereby, they only cease to receive part of their writes. The amount of writes they no longer receive depends, among other things, on the applications access patterns and the compression ratio of the blocks. Moreover, these writes are not evenly distributed among the other frames in the cache. They are only distributed among some of the frames that belong to the same set: those whose effective capacity is larger than the one of the degraded frame.

%En este trabajo proponemos un nuevo procedimiento de pronóstico de la evolución temporal en la capacidad efectiva de una NV-LLC y en las prestaciones del sistema que tiene en cuenta todo lo anterior y que está basado en simulación-predicción.

%A continuación, explicaremos cuál es el mecanismo de compresión que vamos a utilizar en nuestro trabajo junto con algunas consideraciones para su implementación. Después explicaremos nuestro procedimiento de pronóstico para una NV-LLC primero con Block-Disabling y después lo extenderemos para una NV-LLC con compresión.
